Efficient Solution of Point-Line Absolute Pose

We revisit certain problems of pose estimation based on 3D--2D correspondences between features which may be points or lines. Specifically, we address the two previously-studied minimal problems of estimating camera extrinsics from $p \in \{ 1, 2 \}$ point--point correspondences and $l=3-p$ line--line correspondences. To the best of our knowledge, all of the previously-known practical solutions to these problems required computing the roots of degree $\ge 4$ (univariate) polynomials when $p=2$, or degree $\ge 8$ polynomials when $p=1.$ We describe and implement two elementary solutions which reduce the degrees of the needed polynomials from $4$ to $2$ and from $8$ to $4$, respectively. We show experimentally that the resulting solvers are numerically stable and fast: when compared to the previous state-of-the art, we may obtain nearly an order of magnitude speedup. The code is available at \url{https://github.com/petrhruby97/efficient\_absolute}

==> plot/rotation_stability.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.30\columnwidth,
at={(0in,0.389in)},
scale only axis,
xmin=1e-18,
xmax=1e-6,
xlabel style={font=\color{white!15!black}},
xlabel={$\log_{10}$ of rotation error},
label style={font=\small},
title={Rotation stability},
ymin=0,
ymax=15000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
ylabel style={yshift=-0.15in},
ylabel={Frequency},
grid=both,
legend style={at={(1.1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=2
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!90!black,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 1.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 1.000000000000000000e+00 \\
2.112387523010191339e-17 1.500000000000000000e+01 \\
3.363518305757538773e-17 3.300000000000000000e+01 \\
5.355672323345495142e-17 1.570000000000000000e+02 \\
8.527744887236158874e-17 5.580000000000000000e+02 \\
1.357858144994860945e-16 1.780000000000000000e+03 \\
2.162094160073369917e-16 4.706000000000000000e+03 \\
3.442665328668091825e-16 9.266000000000000000e+03 \\
5.481696766070164072e-16 1.276600000000000000e+04 \\
8.728411438927041396e-16 1.332500000000000000e+04 \\
1.389809934740506974e-15 1.210700000000000000e+04 \\
2.212970445101814396e-15 1.030500000000000000e+04 \\
3.523674761908000768e-15 8.314000000000000000e+03 \\
5.610686692716371794e-15 6.453000000000000000e+03 \\
8.933799879640136013e-15 5.008000000000000000e+03 \\
1.422513582750370943e-14 3.840000000000000000e+03 \\
2.265043901107404506e-14 2.808000000000000000e+03 \\
3.606590429895506242e-14 2.183000000000000000e+03 \\
5.742711884151258954e-14 1.587000000000000000e+03 \\
9.144021320249447826e-14 1.137000000000000000e+03 \\
1.455986781017730823e-13 8.530000000000000000e+02 \\
2.318342698746614212e-13 6.080000000000000000e+02 \\
3.691457188282192061e-13 4.850000000000000000e+02 \\
5.877843763257023817e-13 3.830000000000000000e+02 \\
9.359189486181407799e-13 3.120000000000000000e+02 \\
1.490247637846552614e-12 2.090000000000000000e+02 \\
2.372895671560269633e-12 1.590000000000000000e+02 \\
3.778320948218980523e-12 1.420000000000000000e+02 \\
6.016155433569283648e-12 9.300000000000000000e+01 \\
9.579420778937883812e-12 9.200000000000000000e+01 \\
1.525314687647692826e-11 5.500000000000000000e+01 \\
2.428732331571860646e-11 6.200000000000000000e+01 \\
3.867228701193063528e-11 3.200000000000000000e+01 \\
6.157721718824541940e-11 2.400000000000000000e+01 \\
9.804834339067063717e-11 2.700000000000000000e+01 \\
1.561206900965634076e-10 2.300000000000000000e+01 \\
2.485882885252948555e-10 2.300000000000000000e+01 \\
3.958228544449383214e-10 1.600000000000000000e+01 \\
6.302619203438316061e-10 8.000000000000000000e+00 \\
1.003555211061595491e-09 1.100000000000000000e+01 \\
1.597943694741166071e-09 7.000000000000000000e+00 \\
2.544378249864251924e-09 7.000000000000000000e+00 \\
4.051369707010175105e-09 4.000000000000000000e+00 \\
6.450926273935649569e-09 5.000000000000000000e+00 \\
1.027169890709968382e-08 2.000000000000000000e+00 \\
1.635544942815531977e-08 2.000000000000000000e+00 \\
2.604250070181215253e-08 3.000000000000000000e+00 \\
4.146702576306885557e-08 0.000000000000000000e+00 \\
6.602723161356621264e-08 1.000000000000000000e+00 \\
1.051340247902284045e-07 2.000000000000000000e+00 \\
1.674030986681766912e-07 0.000000000000000000e+00 \\
2.665530735613191436e-07 0.000000000000000000e+00 \\
4.244278725438702794e-07 0.000000000000000000e+00 \\
6.758091984659704700e-07 0.000000000000000000e+00 \\
1.076079358299001186e-06 0.000000000000000000e+00 \\
1.713422646489025329e-06 0.000000000000000000e+00 \\
2.728253397725427844e-06 0.000000000000000000e+00 \\
4.344150941072567507e-06 0.000000000000000000e+00 \\
6.917116795146369262e-06 0.000000000000000000e+00 \\
1.101400605244225566e-05 0.000000000000000000e+00 \\
1.753741232305847315e-05 0.000000000000000000e+00 \\
2.792451988173399519e-05 0.000000000000000000e+00 \\
4.446373251999624366e-05 0.000000000000000000e+00 \\
7.079883621931085927e-05 0.000000000000000000e+00 \\
1.127317687005828983e-04 0.000000000000000000e+00 \\
1.795008555648457756e-04 0.000000000000000000e+00 \\
2.858161237059084073e-04 0.000000000000000000e+00 \\
4.551000958363674910e-04 0.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 our}


\addplot [color=red,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 5.000000000000000000e+00 \\
3.363518305757538773e-17 7.000000000000000000e+00 \\
5.355672323345495142e-17 4.400000000000000000e+01 \\
8.527744887236158874e-17 1.870000000000000000e+02 \\
1.357858144994860945e-16 5.380000000000000000e+02 \\
2.162094160073369917e-16 1.650000000000000000e+03 \\
3.442665328668091825e-16 3.875000000000000000e+03 \\
5.481696766070164072e-16 6.412000000000000000e+03 \\
8.728411438927041396e-16 8.003000000000000000e+03 \\
1.389809934740506974e-15 8.195000000000000000e+03 \\
2.212970445101814396e-15 7.978000000000000000e+03 \\
3.523674761908000768e-15 7.318000000000000000e+03 \\
5.610686692716371794e-15 6.539000000000000000e+03 \\
8.933799879640136013e-15 5.865000000000000000e+03 \\
1.422513582750370943e-14 5.027000000000000000e+03 \\
2.265043901107404506e-14 4.322000000000000000e+03 \\
3.606590429895506242e-14 3.930000000000000000e+03 \\
5.742711884151258954e-14 3.368000000000000000e+03 \\
9.144021320249447826e-14 3.112000000000000000e+03 \\
1.455986781017730823e-13 2.839000000000000000e+03 \\
2.318342698746614212e-13 2.529000000000000000e+03 \\
3.691457188282192061e-13 2.249000000000000000e+03 \\
5.877843763257023817e-13 2.077000000000000000e+03 \\
9.359189486181407799e-13 1.861000000000000000e+03 \\
1.490247637846552614e-12 1.703000000000000000e+03 \\
2.372895671560269633e-12 1.431000000000000000e+03 \\
3.778320948218980523e-12 1.303000000000000000e+03 \\
6.016155433569283648e-12 1.106000000000000000e+03 \\
9.579420778937883812e-12 9.660000000000000000e+02 \\
1.525314687647692826e-11 8.040000000000000000e+02 \\
2.428732331571860646e-11 7.350000000000000000e+02 \\
3.867228701193063528e-11 6.600000000000000000e+02 \\
6.157721718824541940e-11 6.210000000000000000e+02 \\
9.804834339067063717e-11 5.010000000000000000e+02 \\
1.561206900965634076e-10 4.300000000000000000e+02 \\
2.485882885252948555e-10 3.840000000000000000e+02 \\
3.958228544449383214e-10 3.090000000000000000e+02 \\
6.302619203438316061e-10 2.660000000000000000e+02 \\
1.003555211061595491e-09 1.910000000000000000e+02 \\
1.597943694741166071e-09 1.630000000000000000e+02 \\
2.544378249864251924e-09 1.330000000000000000e+02 \\
4.051369707010175105e-09 1.050000000000000000e+02 \\
6.450926273935649569e-09 7.800000000000000000e+01 \\
1.027169890709968382e-08 6.200000000000000000e+01 \\
1.635544942815531977e-08 3.600000000000000000e+01 \\
2.604250070181215253e-08 2.900000000000000000e+01 \\
4.146702576306885557e-08 2.100000000000000000e+01 \\
6.602723161356621264e-08 9.000000000000000000e+00 \\
1.051340247902284045e-07 7.000000000000000000e+00 \\
1.674030986681766912e-07 4.000000000000000000e+00 \\
2.665530735613191436e-07 4.000000000000000000e+00 \\
4.244278725438702794e-07 1.000000000000000000e+00 \\
6.758091984659704700e-07 2.000000000000000000e+00 \\
1.076079358299001186e-06 2.000000000000000000e+00 \\
1.713422646489025329e-06 0.000000000000000000e+00 \\
2.728253397725427844e-06 2.000000000000000000e+00 \\
4.344150941072567507e-06 0.000000000000000000e+00 \\
6.917116795146369262e-06 0.000000000000000000e+00 \\
1.101400605244225566e-05 0.000000000000000000e+00 \\
1.753741232305847315e-05 0.000000000000000000e+00 \\
2.792451988173399519e-05 0.000000000000000000e+00 \\
4.446373251999624366e-05 0.000000000000000000e+00 \\
7.079883621931085927e-05 0.000000000000000000e+00 \\
1.127317687005828983e-04 0.000000000000000000e+00 \\
1.795008555648457756e-04 0.000000000000000000e+00 \\
2.858161237059084073e-04 0.000000000000000000e+00 \\
4.551000958363674910e-04 0.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 1.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 1.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 3Q3}

\addplot [dashed,color=red,line width=2pt, mark options={solid, magenta}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 2.000000000000000000e+00 \\
5.355672323345495142e-17 1.000000000000000000e+01 \\
8.527744887236158874e-17 4.000000000000000000e+01 \\
1.357858144994860945e-16 1.360000000000000000e+02 \\
2.162094160073369917e-16 4.790000000000000000e+02 \\
3.442665328668091825e-16 1.214000000000000000e+03 \\
5.481696766070164072e-16 2.437000000000000000e+03 \\
8.728411438927041396e-16 3.939000000000000000e+03 \\
1.389809934740506974e-15 5.624000000000000000e+03 \\
2.212970445101814396e-15 6.757000000000000000e+03 \\
3.523674761908000768e-15 7.672000000000000000e+03 \\
5.610686692716371794e-15 8.312000000000000000e+03 \\
8.933799879640136013e-15 8.352000000000000000e+03 \\
1.422513582750370943e-14 7.933000000000000000e+03 \\
2.265043901107404506e-14 7.232000000000000000e+03 \\
3.606590429895506242e-14 6.327000000000000000e+03 \\
5.742711884151258954e-14 5.360000000000000000e+03 \\
9.144021320249447826e-14 4.670000000000000000e+03 \\
1.455986781017730823e-13 4.059000000000000000e+03 \\
2.318342698746614212e-13 3.472000000000000000e+03 \\
3.691457188282192061e-13 2.887000000000000000e+03 \\
5.877843763257023817e-13 2.351000000000000000e+03 \\
9.359189486181407799e-13 1.908000000000000000e+03 \\
1.490247637846552614e-12 1.645000000000000000e+03 \\
2.372895671560269633e-12 1.416000000000000000e+03 \\
3.778320948218980523e-12 1.173000000000000000e+03 \\
6.016155433569283648e-12 8.970000000000000000e+02 \\
9.579420778937883812e-12 6.650000000000000000e+02 \\
1.525314687647692826e-11 6.160000000000000000e+02 \\
2.428732331571860646e-11 4.700000000000000000e+02 \\
3.867228701193063528e-11 3.600000000000000000e+02 \\
6.157721718824541940e-11 3.320000000000000000e+02 \\
9.804834339067063717e-11 2.860000000000000000e+02 \\
1.561206900965634076e-10 1.970000000000000000e+02 \\
2.485882885252948555e-10 1.620000000000000000e+02 \\
3.958228544449383214e-10 1.260000000000000000e+02 \\
6.302619203438316061e-10 1.030000000000000000e+02 \\
1.003555211061595491e-09 8.900000000000000000e+01 \\
1.597943694741166071e-09 6.600000000000000000e+01 \\
2.544378249864251924e-09 4.000000000000000000e+01 \\
4.051369707010175105e-09 3.700000000000000000e+01 \\
6.450926273935649569e-09 3.400000000000000000e+01 \\
1.027169890709968382e-08 2.400000000000000000e+01 \\
1.635544942815531977e-08 1.600000000000000000e+01 \\
2.604250070181215253e-08 1.100000000000000000e+01 \\
4.146702576306885557e-08 1.800000000000000000e+01 \\
6.602723161356621264e-08 9.000000000000000000e+00 \\
1.051340247902284045e-07 1.700000000000000000e+01 \\
1.674030986681766912e-07 4.000000000000000000e+00 \\
2.665530735613191436e-07 4.000000000000000000e+00 \\
4.244278725438702794e-07 2.000000000000000000e+00 \\
6.758091984659704700e-07 1.000000000000000000e+00 \\
1.076079358299001186e-06 0.000000000000000000e+00 \\
1.713422646489025329e-06 2.000000000000000000e+00 \\
2.728253397725427844e-06 1.000000000000000000e+00 \\
4.344150941072567507e-06 1.000000000000000000e+00 \\
6.917116795146369262e-06 0.000000000000000000e+00 \\
1.101400605244225566e-05 0.000000000000000000e+00 \\
1.753741232305847315e-05 1.000000000000000000e+00 \\
2.792451988173399519e-05 0.000000000000000000e+00 \\
4.446373251999624366e-05 1.000000000000000000e+00 \\
7.079883621931085927e-05 0.000000000000000000e+00 \\
1.127317687005828983e-04 0.000000000000000000e+00 \\
1.795008555648457756e-04 0.000000000000000000e+00 \\
2.858161237059084073e-04 0.000000000000000000e+00 \\
4.551000958363674910e-04 1.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 \textit{Ram.}+SVD}

\addplot [dashed,color=brown,line width=2pt, mark options={solid, magenta}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 1.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 1.000000000000000000e+01 \\
5.355672323345495142e-17 2.300000000000000000e+01 \\
8.527744887236158874e-17 8.500000000000000000e+01 \\
1.357858144994860945e-16 2.570000000000000000e+02 \\
2.162094160073369917e-16 7.270000000000000000e+02 \\
3.442665328668091825e-16 1.816000000000000000e+03 \\
5.481696766070164072e-16 3.146000000000000000e+03 \\
8.728411438927041396e-16 4.554000000000000000e+03 \\
1.389809934740506974e-15 5.781000000000000000e+03 \\
2.212970445101814396e-15 6.915000000000000000e+03 \\
3.523674761908000768e-15 7.752000000000000000e+03 \\
5.610686692716371794e-15 8.188000000000000000e+03 \\
8.933799879640136013e-15 8.134000000000000000e+03 \\
1.422513582750370943e-14 7.539000000000000000e+03 \\
2.265043901107404506e-14 6.626000000000000000e+03 \\
3.606590429895506242e-14 5.582000000000000000e+03 \\
5.742711884151258954e-14 4.729000000000000000e+03 \\
9.144021320249447826e-14 4.059000000000000000e+03 \\
1.455986781017730823e-13 3.486000000000000000e+03 \\
2.318342698746614212e-13 3.159000000000000000e+03 \\
3.691457188282192061e-13 2.683000000000000000e+03 \\
5.877843763257023817e-13 2.268000000000000000e+03 \\
9.359189486181407799e-13 1.901000000000000000e+03 \\
1.490247637846552614e-12 1.673000000000000000e+03 \\
2.372895671560269633e-12 1.444000000000000000e+03 \\
3.778320948218980523e-12 1.220000000000000000e+03 \\
6.016155433569283648e-12 1.095000000000000000e+03 \\
9.579420778937883812e-12 8.780000000000000000e+02 \\
1.525314687647692826e-11 7.270000000000000000e+02 \\
2.428732331571860646e-11 5.760000000000000000e+02 \\
3.867228701193063528e-11 4.990000000000000000e+02 \\
6.157721718824541940e-11 4.240000000000000000e+02 \\
9.804834339067063717e-11 3.850000000000000000e+02 \\
1.561206900965634076e-10 2.820000000000000000e+02 \\
2.485882885252948555e-10 2.360000000000000000e+02 \\
3.958228544449383214e-10 1.880000000000000000e+02 \\
6.302619203438316061e-10 1.700000000000000000e+02 \\
1.003555211061595491e-09 1.380000000000000000e+02 \\
1.597943694741166071e-09 1.060000000000000000e+02 \\
2.544378249864251924e-09 9.000000000000000000e+01 \\
4.051369707010175105e-09 8.100000000000000000e+01 \\
6.450926273935649569e-09 5.300000000000000000e+01 \\
1.027169890709968382e-08 6.000000000000000000e+01 \\
1.635544942815531977e-08 4.000000000000000000e+01 \\
2.604250070181215253e-08 2.400000000000000000e+01 \\
4.146702576306885557e-08 3.200000000000000000e+01 \\
6.602723161356621264e-08 2.200000000000000000e+01 \\
1.051340247902284045e-07 2.600000000000000000e+01 \\
1.674030986681766912e-07 1.200000000000000000e+01 \\
2.665530735613191436e-07 1.100000000000000000e+01 \\
4.244278725438702794e-07 1.400000000000000000e+01 \\
6.758091984659704700e-07 1.000000000000000000e+01 \\
1.076079358299001186e-06 8.000000000000000000e+00 \\
1.713422646489025329e-06 8.000000000000000000e+00 \\
2.728253397725427844e-06 9.000000000000000000e+00 \\
4.344150941072567507e-06 1.000000000000000000e+00 \\
6.917116795146369262e-06 1.000000000000000000e+00 \\
1.101400605244225566e-05 5.000000000000000000e+00 \\
1.753741232305847315e-05 3.000000000000000000e+00 \\
2.792451988173399519e-05 3.000000000000000000e+00 \\
4.446373251999624366e-05 5.000000000000000000e+00 \\
7.079883621931085927e-05 2.000000000000000000e+00 \\
1.127317687005828983e-04 4.000000000000000000e+00 \\
1.795008555648457756e-04 5.000000000000000000e+00 \\
2.858161237059084073e-04 6.000000000000000000e+00 \\
4.551000958363674910e-04 1.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 1.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 1.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 \textit{Ram.}+LU}

\addplot [color=cyan,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 1.000000000000000000e+00 \\
1.326640928259833440e-17 1.000000000000000000e+00 \\
2.112387523010191339e-17 1.000000000000000000e+00 \\
3.363518305757538773e-17 1.300000000000000000e+01 \\
5.355672323345495142e-17 4.700000000000000000e+01 \\
8.527744887236158874e-17 1.790000000000000000e+02 \\
1.357858144994860945e-16 6.090000000000000000e+02 \\
2.162094160073369917e-16 1.720000000000000000e+03 \\
3.442665328668091825e-16 3.832000000000000000e+03 \\
5.481696766070164072e-16 6.319000000000000000e+03 \\
8.728411438927041396e-16 8.464000000000000000e+03 \\
1.389809934740506974e-15 9.593000000000000000e+03 \\
2.212970445101814396e-15 9.759000000000000000e+03 \\
3.523674761908000768e-15 9.350000000000000000e+03 \\
5.610686692716371794e-15 8.473000000000000000e+03 \\
8.933799879640136013e-15 7.410000000000000000e+03 \\
1.422513582750370943e-14 6.308000000000000000e+03 \\
2.265043901107404506e-14 5.213000000000000000e+03 \\
3.606590429895506242e-14 4.373000000000000000e+03 \\
5.742711884151258954e-14 3.441000000000000000e+03 \\
9.144021320249447826e-14 2.771000000000000000e+03 \\
1.455986781017730823e-13 2.304000000000000000e+03 \\
2.318342698746614212e-13 1.917000000000000000e+03 \\
3.691457188282192061e-13 1.470000000000000000e+03 \\
5.877843763257023817e-13 1.223000000000000000e+03 \\
9.359189486181407799e-13 9.800000000000000000e+02 \\
1.490247637846552614e-12 7.900000000000000000e+02 \\
2.372895671560269633e-12 6.330000000000000000e+02 \\
3.778320948218980523e-12 5.320000000000000000e+02 \\
6.016155433569283648e-12 4.090000000000000000e+02 \\
9.579420778937883812e-12 3.330000000000000000e+02 \\
1.525314687647692826e-11 2.490000000000000000e+02 \\
2.428732331571860646e-11 2.400000000000000000e+02 \\
3.867228701193063528e-11 1.890000000000000000e+02 \\
6.157721718824541940e-11 1.460000000000000000e+02 \\
9.804834339067063717e-11 1.150000000000000000e+02 \\
1.561206900965634076e-10 1.190000000000000000e+02 \\
2.485882885252948555e-10 7.300000000000000000e+01 \\
3.958228544449383214e-10 6.500000000000000000e+01 \\
6.302619203438316061e-10 4.600000000000000000e+01 \\
1.003555211061595491e-09 5.700000000000000000e+01 \\
1.597943694741166071e-09 3.500000000000000000e+01 \\
2.544378249864251924e-09 3.700000000000000000e+01 \\
4.051369707010175105e-09 2.600000000000000000e+01 \\
6.450926273935649569e-09 2.200000000000000000e+01 \\
1.027169890709968382e-08 1.600000000000000000e+01 \\
1.635544942815531977e-08 9.000000000000000000e+00 \\
2.604250070181215253e-08 1.800000000000000000e+01 \\
4.146702576306885557e-08 1.600000000000000000e+01 \\
6.602723161356621264e-08 1.100000000000000000e+01 \\
1.051340247902284045e-07 1.000000000000000000e+01 \\
1.674030986681766912e-07 6.000000000000000000e+00 \\
2.665530735613191436e-07 8.000000000000000000e+00 \\
4.244278725438702794e-07 0.000000000000000000e+00 \\
6.758091984659704700e-07 5.000000000000000000e+00 \\
1.076079358299001186e-06 4.000000000000000000e+00 \\
1.713422646489025329e-06 0.000000000000000000e+00 \\
2.728253397725427844e-06 1.000000000000000000e+00 \\
4.344150941072567507e-06 1.000000000000000000e+00 \\
6.917116795146369262e-06 0.000000000000000000e+00 \\
1.101400605244225566e-05 0.000000000000000000e+00 \\
1.753741232305847315e-05 2.000000000000000000e+00 \\
2.792451988173399519e-05 0.000000000000000000e+00 \\
4.446373251999624366e-05 1.000000000000000000e+00 \\
7.079883621931085927e-05 1.000000000000000000e+00 \\
1.127317687005828983e-04 1.000000000000000000e+00 \\
1.795008555648457756e-04 0.000000000000000000e+00 \\
2.858161237059084073e-04 0.000000000000000000e+00 \\
4.551000958363674910e-04 0.000000000000000000e+00 \\
7.246480518481307606e-04 2.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 1.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P1L2 our}


\addplot [dashed,color=black,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 1.000000000000000000e+00 \\
2.112387523010191339e-17 4.000000000000000000e+00 \\
3.363518305757538773e-17 6.000000000000000000e+00 \\
5.355672323345495142e-17 4.100000000000000000e+01 \\
8.527744887236158874e-17 1.130000000000000000e+02 \\
1.357858144994860945e-16 4.270000000000000000e+02 \\
2.162094160073369917e-16 1.356000000000000000e+03 \\
3.442665328668091825e-16 3.369000000000000000e+03 \\
5.481696766070164072e-16 5.723000000000000000e+03 \\
8.728411438927041396e-16 7.801000000000000000e+03 \\
1.389809934740506974e-15 8.153000000000000000e+03 \\
2.212970445101814396e-15 8.180000000000000000e+03 \\
3.523674761908000768e-15 7.326000000000000000e+03 \\
5.610686692716371794e-15 6.809000000000000000e+03 \\
8.933799879640136013e-15 5.965000000000000000e+03 \\
1.422513582750370943e-14 5.286000000000000000e+03 \\
2.265043901107404506e-14 4.520000000000000000e+03 \\
3.606590429895506242e-14 3.984000000000000000e+03 \\
5.742711884151258954e-14 3.486000000000000000e+03 \\
9.144021320249447826e-14 3.160000000000000000e+03 \\
1.455986781017730823e-13 2.828000000000000000e+03 \\
2.318342698746614212e-13 2.494000000000000000e+03 \\
3.691457188282192061e-13 2.246000000000000000e+03 \\
5.877843763257023817e-13 2.099000000000000000e+03 \\
9.359189486181407799e-13 1.902000000000000000e+03 \\
1.490247637846552614e-12 1.609000000000000000e+03 \\
2.372895671560269633e-12 1.516000000000000000e+03 \\
3.778320948218980523e-12 1.316000000000000000e+03 \\
6.016155433569283648e-12 1.188000000000000000e+03 \\
9.579420778937883812e-12 1.008000000000000000e+03 \\
1.525314687647692826e-11 8.950000000000000000e+02 \\
2.428732331571860646e-11 8.430000000000000000e+02 \\
3.867228701193063528e-11 7.630000000000000000e+02 \\
6.157721718824541940e-11 6.610000000000000000e+02 \\
9.804834339067063717e-11 5.570000000000000000e+02 \\
1.561206900965634076e-10 4.750000000000000000e+02 \\
2.485882885252948555e-10 4.430000000000000000e+02 \\
3.958228544449383214e-10 3.340000000000000000e+02 \\
6.302619203438316061e-10 2.820000000000000000e+02 \\
1.003555211061595491e-09 2.200000000000000000e+02 \\
1.597943694741166071e-09 1.830000000000000000e+02 \\
2.544378249864251924e-09 1.130000000000000000e+02 \\
4.051369707010175105e-09 1.060000000000000000e+02 \\
6.450926273935649569e-09 5.400000000000000000e+01 \\
1.027169890709968382e-08 5.600000000000000000e+01 \\
1.635544942815531977e-08 2.400000000000000000e+01 \\
2.604250070181215253e-08 2.700000000000000000e+01 \\
4.146702576306885557e-08 1.000000000000000000e+01 \\
6.602723161356621264e-08 6.000000000000000000e+00 \\
1.051340247902284045e-07 7.000000000000000000e+00 \\
1.674030986681766912e-07 3.000000000000000000e+00 \\
2.665530735613191436e-07 4.000000000000000000e+00 \\
4.244278725438702794e-07 2.000000000000000000e+00 \\
6.758091984659704700e-07 2.000000000000000000e+00 \\
1.076079358299001186e-06 1.000000000000000000e+00 \\
1.713422646489025329e-06 2.000000000000000000e+00 \\
2.728253397725427844e-06 1.000000000000000000e+00 \\
4.344150941072567507e-06 2.000000000000000000e+00 \\
6.917116795146369262e-06 0.000000000000000000e+00 \\
1.101400605244225566e-05 1.000000000000000000e+00 \\
1.753741232305847315e-05 1.000000000000000000e+00 \\
2.792451988173399519e-05 1.000000000000000000e+00 \\
4.446373251999624366e-05 0.000000000000000000e+00 \\
7.079883621931085927e-05 0.000000000000000000e+00 \\
1.127317687005828983e-04 0.000000000000000000e+00 \\
1.795008555648457756e-04 1.000000000000000000e+00 \\
2.858161237059084073e-04 0.000000000000000000e+00 \\
4.551000958363674910e-04 0.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 1.000000000000000000e+00 \\
3.064712609718931446e-01 2.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 1.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P1L2 3Q3}



%\legend{}

\end{axis}

==> plot/translation_stability.tex <==
\begin{axis}[%
xmode=log,
width=0.35\columnwidth,
height=0.30\columnwidth,
at={(1.5in,0.389in)},
scale only axis,
xmin=1e-18,
xmax=1e-6,
xlabel style={font=\color{white!15!black}},
xlabel={$\log_{10}$ of translation error},
label style={font=\small},
title={Translation stability},
ymin=0,
ymax=15000,
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
grid=both,
legend style={at={(1.73,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=green!90!black,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 1.000000000000000000e+00 \\
5.355672323345495142e-17 3.000000000000000000e+00 \\
8.527744887236158874e-17 3.000000000000000000e+00 \\
1.357858144994860945e-16 8.000000000000000000e+00 \\
2.162094160073369917e-16 5.500000000000000000e+01 \\
3.442665328668091825e-16 1.580000000000000000e+02 \\
5.481696766070164072e-16 5.150000000000000000e+02 \\
8.728411438927041396e-16 1.284000000000000000e+03 \\
1.389809934740506974e-15 2.775000000000000000e+03 \\
2.212970445101814396e-15 4.946000000000000000e+03 \\
3.523674761908000768e-15 7.420000000000000000e+03 \\
5.610686692716371794e-15 8.907000000000000000e+03 \\
8.933799879640136013e-15 1.004900000000000000e+04 \\
1.422513582750370943e-14 1.009400000000000000e+04 \\
2.265043901107404506e-14 9.622000000000000000e+03 \\
3.606590429895506242e-14 8.549000000000000000e+03 \\
5.742711884151258954e-14 7.204000000000000000e+03 \\
9.144021320249447826e-14 6.187000000000000000e+03 \\
1.455986781017730823e-13 4.856000000000000000e+03 \\
2.318342698746614212e-13 3.994000000000000000e+03 \\
3.691457188282192061e-13 3.040000000000000000e+03 \\
5.877843763257023817e-13 2.386000000000000000e+03 \\
9.359189486181407799e-13 1.814000000000000000e+03 \\
1.490247637846552614e-12 1.397000000000000000e+03 \\
2.372895671560269633e-12 1.164000000000000000e+03 \\
3.778320948218980523e-12 7.920000000000000000e+02 \\
6.016155433569283648e-12 6.040000000000000000e+02 \\
9.579420778937883812e-12 4.640000000000000000e+02 \\
1.525314687647692826e-11 3.850000000000000000e+02 \\
2.428732331571860646e-11 3.180000000000000000e+02 \\
3.867228701193063528e-11 2.110000000000000000e+02 \\
6.157721718824541940e-11 1.640000000000000000e+02 \\
9.804834339067063717e-11 1.380000000000000000e+02 \\
1.561206900965634076e-10 9.300000000000000000e+01 \\
2.485882885252948555e-10 8.200000000000000000e+01 \\
3.958228544449383214e-10 6.600000000000000000e+01 \\
6.302619203438316061e-10 5.400000000000000000e+01 \\
1.003555211061595491e-09 4.300000000000000000e+01 \\
1.597943694741166071e-09 2.500000000000000000e+01 \\
2.544378249864251924e-09 2.900000000000000000e+01 \\
4.051369707010175105e-09 1.900000000000000000e+01 \\
6.450926273935649569e-09 1.800000000000000000e+01 \\
1.027169890709968382e-08 1.200000000000000000e+01 \\
1.635544942815531977e-08 1.200000000000000000e+01 \\
2.604250070181215253e-08 1.200000000000000000e+01 \\
4.146702576306885557e-08 5.000000000000000000e+00 \\
6.602723161356621264e-08 5.000000000000000000e+00 \\
1.051340247902284045e-07 4.000000000000000000e+00 \\
1.674030986681766912e-07 3.000000000000000000e+00 \\
2.665530735613191436e-07 4.000000000000000000e+00 \\
4.244278725438702794e-07 1.000000000000000000e+00 \\
6.758091984659704700e-07 2.000000000000000000e+00 \\
1.076079358299001186e-06 1.000000000000000000e+00 \\
1.713422646489025329e-06 1.000000000000000000e+00 \\
2.728253397725427844e-06 0.000000000000000000e+00 \\
4.344150941072567507e-06 0.000000000000000000e+00 \\
6.917116795146369262e-06 1.000000000000000000e+00 \\
1.101400605244225566e-05 0.000000000000000000e+00 \\
1.753741232305847315e-05 0.000000000000000000e+00 \\
2.792451988173399519e-05 1.000000000000000000e+00 \\
4.446373251999624366e-05 0.000000000000000000e+00 \\
7.079883621931085927e-05 0.000000000000000000e+00 \\
1.127317687005828983e-04 0.000000000000000000e+00 \\
1.795008555648457756e-04 0.000000000000000000e+00 \\
2.858161237059084073e-04 0.000000000000000000e+00 \\
4.551000958363674910e-04 0.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 our}


\addplot [color=red,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 0.000000000000000000e+00 \\
5.355672323345495142e-17 1.000000000000000000e+00 \\
8.527744887236158874e-17 0.000000000000000000e+00 \\
1.357858144994860945e-16 3.000000000000000000e+00 \\
2.162094160073369917e-16 9.000000000000000000e+00 \\
3.442665328668091825e-16 4.600000000000000000e+01 \\
5.481696766070164072e-16 1.230000000000000000e+02 \\
8.728411438927041396e-16 4.270000000000000000e+02 \\
1.389809934740506974e-15 9.580000000000000000e+02 \\
2.212970445101814396e-15 1.989000000000000000e+03 \\
3.523674761908000768e-15 3.307000000000000000e+03 \\
5.610686692716371794e-15 4.546000000000000000e+03 \\
8.933799879640136013e-15 5.529000000000000000e+03 \\
1.422513582750370943e-14 6.390000000000000000e+03 \\
2.265043901107404506e-14 6.600000000000000000e+03 \\
3.606590429895506242e-14 6.596000000000000000e+03 \\
5.742711884151258954e-14 6.287000000000000000e+03 \\
9.144021320249447826e-14 6.082000000000000000e+03 \\
1.455986781017730823e-13 5.363000000000000000e+03 \\
2.318342698746614212e-13 4.820000000000000000e+03 \\
3.691457188282192061e-13 4.435000000000000000e+03 \\
5.877843763257023817e-13 3.847000000000000000e+03 \\
9.359189486181407799e-13 3.595000000000000000e+03 \\
1.490247637846552614e-12 3.302000000000000000e+03 \\
2.372895671560269633e-12 2.963000000000000000e+03 \\
3.778320948218980523e-12 2.642000000000000000e+03 \\
6.016155433569283648e-12 2.394000000000000000e+03 \\
9.579420778937883812e-12 2.130000000000000000e+03 \\
1.525314687647692826e-11 1.943000000000000000e+03 \\
2.428732331571860646e-11 1.785000000000000000e+03 \\
3.867228701193063528e-11 1.523000000000000000e+03 \\
6.157721718824541940e-11 1.445000000000000000e+03 \\
9.804834339067063717e-11 1.208000000000000000e+03 \\
1.561206900965634076e-10 1.068000000000000000e+03 \\
2.485882885252948555e-10 9.560000000000000000e+02 \\
3.958228544449383214e-10 8.960000000000000000e+02 \\
6.302619203438316061e-10 7.910000000000000000e+02 \\
1.003555211061595491e-09 6.580000000000000000e+02 \\
1.597943694741166071e-09 5.530000000000000000e+02 \\
2.544378249864251924e-09 5.350000000000000000e+02 \\
4.051369707010175105e-09 4.790000000000000000e+02 \\
6.450926273935649569e-09 3.580000000000000000e+02 \\
1.027169890709968382e-08 2.950000000000000000e+02 \\
1.635544942815531977e-08 2.340000000000000000e+02 \\
2.604250070181215253e-08 2.060000000000000000e+02 \\
4.146702576306885557e-08 1.480000000000000000e+02 \\
6.602723161356621264e-08 1.370000000000000000e+02 \\
1.051340247902284045e-07 1.040000000000000000e+02 \\
1.674030986681766912e-07 7.300000000000000000e+01 \\
2.665530735613191436e-07 6.500000000000000000e+01 \\
4.244278725438702794e-07 4.700000000000000000e+01 \\
6.758091984659704700e-07 2.900000000000000000e+01 \\
1.076079358299001186e-06 2.200000000000000000e+01 \\
1.713422646489025329e-06 1.900000000000000000e+01 \\
2.728253397725427844e-06 9.000000000000000000e+00 \\
4.344150941072567507e-06 9.000000000000000000e+00 \\
6.917116795146369262e-06 1.000000000000000000e+00 \\
1.101400605244225566e-05 5.000000000000000000e+00 \\
1.753741232305847315e-05 4.000000000000000000e+00 \\
2.792451988173399519e-05 2.000000000000000000e+00 \\
4.446373251999624366e-05 0.000000000000000000e+00 \\
7.079883621931085927e-05 1.000000000000000000e+00 \\
1.127317687005828983e-04 2.000000000000000000e+00 \\
1.795008555648457756e-04 1.000000000000000000e+00 \\
2.858161237059084073e-04 2.000000000000000000e+00 \\
4.551000958363674910e-04 0.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 1.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 2.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 3Q3}

\addplot [dashed,color=red,line width=2pt, mark options={solid, magenta}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 0.000000000000000000e+00 \\
5.355672323345495142e-17 0.000000000000000000e+00 \\
8.527744887236158874e-17 0.000000000000000000e+00 \\
1.357858144994860945e-16 2.000000000000000000e+00 \\
2.162094160073369917e-16 3.000000000000000000e+00 \\
3.442665328668091825e-16 9.000000000000000000e+00 \\
5.481696766070164072e-16 2.900000000000000000e+01 \\
8.728411438927041396e-16 1.000000000000000000e+02 \\
1.389809934740506974e-15 2.500000000000000000e+02 \\
2.212970445101814396e-15 5.330000000000000000e+02 \\
3.523674761908000768e-15 1.121000000000000000e+03 \\
5.610686692716371794e-15 1.861000000000000000e+03 \\
8.933799879640136013e-15 2.791000000000000000e+03 \\
1.422513582750370943e-14 3.886000000000000000e+03 \\
2.265043901107404506e-14 5.144000000000000000e+03 \\
3.606590429895506242e-14 5.984000000000000000e+03 \\
5.742711884151258954e-14 6.856000000000000000e+03 \\
9.144021320249447826e-14 7.397000000000000000e+03 \\
1.455986781017730823e-13 7.540000000000000000e+03 \\
2.318342698746614212e-13 7.246000000000000000e+03 \\
3.691457188282192061e-13 6.742000000000000000e+03 \\
5.877843763257023817e-13 6.069000000000000000e+03 \\
9.359189486181407799e-13 5.551000000000000000e+03 \\
1.490247637846552614e-12 4.900000000000000000e+03 \\
2.372895671560269633e-12 4.388000000000000000e+03 \\
3.778320948218980523e-12 3.619000000000000000e+03 \\
6.016155433569283648e-12 3.072000000000000000e+03 \\
9.579420778937883812e-12 2.633000000000000000e+03 \\
1.525314687647692826e-11 2.221000000000000000e+03 \\
2.428732331571860646e-11 1.873000000000000000e+03 \\
3.867228701193063528e-11 1.548000000000000000e+03 \\
6.157721718824541940e-11 1.242000000000000000e+03 \\
9.804834339067063717e-11 1.039000000000000000e+03 \\
1.561206900965634076e-10 8.680000000000000000e+02 \\
2.485882885252948555e-10 6.390000000000000000e+02 \\
3.958228544449383214e-10 5.520000000000000000e+02 \\
6.302619203438316061e-10 4.200000000000000000e+02 \\
1.003555211061595491e-09 3.990000000000000000e+02 \\
1.597943694741166071e-09 2.750000000000000000e+02 \\
2.544378249864251924e-09 2.580000000000000000e+02 \\
4.051369707010175105e-09 1.930000000000000000e+02 \\
6.450926273935649569e-09 1.320000000000000000e+02 \\
1.027169890709968382e-08 1.410000000000000000e+02 \\
1.635544942815531977e-08 8.900000000000000000e+01 \\
2.604250070181215253e-08 8.600000000000000000e+01 \\
4.146702576306885557e-08 6.700000000000000000e+01 \\
6.602723161356621264e-08 4.500000000000000000e+01 \\
1.051340247902284045e-07 4.600000000000000000e+01 \\
1.674030986681766912e-07 2.900000000000000000e+01 \\
2.665530735613191436e-07 1.600000000000000000e+01 \\
4.244278725438702794e-07 2.600000000000000000e+01 \\
6.758091984659704700e-07 1.600000000000000000e+01 \\
1.076079358299001186e-06 1.000000000000000000e+01 \\
1.713422646489025329e-06 8.000000000000000000e+00 \\
2.728253397725427844e-06 7.000000000000000000e+00 \\
4.344150941072567507e-06 5.000000000000000000e+00 \\
6.917116795146369262e-06 4.000000000000000000e+00 \\
1.101400605244225566e-05 6.000000000000000000e+00 \\
1.753741232305847315e-05 3.000000000000000000e+00 \\
2.792451988173399519e-05 3.000000000000000000e+00 \\
4.446373251999624366e-05 2.000000000000000000e+00 \\
7.079883621931085927e-05 0.000000000000000000e+00 \\
1.127317687005828983e-04 0.000000000000000000e+00 \\
1.795008555648457756e-04 0.000000000000000000e+00 \\
2.858161237059084073e-04 1.000000000000000000e+00 \\
4.551000958363674910e-04 1.000000000000000000e+00 \\
7.246480518481307606e-04 1.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 1.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 1.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 \textit{Ramalingam} (SVD)}

\addplot [dashed,color=brown,line width=2pt, mark options={solid, magenta}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 0.000000000000000000e+00 \\
5.355672323345495142e-17 0.000000000000000000e+00 \\
8.527744887236158874e-17 0.000000000000000000e+00 \\
1.357858144994860945e-16 1.000000000000000000e+00 \\
2.162094160073369917e-16 5.000000000000000000e+00 \\
3.442665328668091825e-16 1.800000000000000000e+01 \\
5.481696766070164072e-16 6.500000000000000000e+01 \\
8.728411438927041396e-16 1.870000000000000000e+02 \\
1.389809934740506974e-15 4.470000000000000000e+02 \\
2.212970445101814396e-15 8.240000000000000000e+02 \\
3.523674761908000768e-15 1.474000000000000000e+03 \\
5.610686692716371794e-15 2.329000000000000000e+03 \\
8.933799879640136013e-15 3.217000000000000000e+03 \\
1.422513582750370943e-14 4.112000000000000000e+03 \\
2.265043901107404506e-14 5.361000000000000000e+03 \\
3.606590429895506242e-14 6.076000000000000000e+03 \\
5.742711884151258954e-14 6.875000000000000000e+03 \\
9.144021320249447826e-14 7.252000000000000000e+03 \\
1.455986781017730823e-13 7.233000000000000000e+03 \\
2.318342698746614212e-13 6.908000000000000000e+03 \\
3.691457188282192061e-13 6.306000000000000000e+03 \\
5.877843763257023817e-13 5.544000000000000000e+03 \\
9.359189486181407799e-13 4.936000000000000000e+03 \\
1.490247637846552614e-12 4.311000000000000000e+03 \\
2.372895671560269633e-12 3.852000000000000000e+03 \\
3.778320948218980523e-12 3.339000000000000000e+03 \\
6.016155433569283648e-12 2.875000000000000000e+03 \\
9.579420778937883812e-12 2.481000000000000000e+03 \\
1.525314687647692826e-11 2.218000000000000000e+03 \\
2.428732331571860646e-11 1.856000000000000000e+03 \\
3.867228701193063528e-11 1.535000000000000000e+03 \\
6.157721718824541940e-11 1.368000000000000000e+03 \\
9.804834339067063717e-11 1.148000000000000000e+03 \\
1.561206900965634076e-10 9.730000000000000000e+02 \\
2.485882885252948555e-10 8.250000000000000000e+02 \\
3.958228544449383214e-10 6.800000000000000000e+02 \\
6.302619203438316061e-10 5.260000000000000000e+02 \\
1.003555211061595491e-09 4.820000000000000000e+02 \\
1.597943694741166071e-09 4.110000000000000000e+02 \\
2.544378249864251924e-09 3.230000000000000000e+02 \\
4.051369707010175105e-09 2.770000000000000000e+02 \\
6.450926273935649569e-09 2.310000000000000000e+02 \\
1.027169890709968382e-08 1.970000000000000000e+02 \\
1.635544942815531977e-08 1.770000000000000000e+02 \\
2.604250070181215253e-08 1.240000000000000000e+02 \\
4.146702576306885557e-08 1.080000000000000000e+02 \\
6.602723161356621264e-08 7.600000000000000000e+01 \\
1.051340247902284045e-07 8.000000000000000000e+01 \\
1.674030986681766912e-07 5.600000000000000000e+01 \\
2.665530735613191436e-07 4.800000000000000000e+01 \\
4.244278725438702794e-07 3.900000000000000000e+01 \\
6.758091984659704700e-07 2.100000000000000000e+01 \\
1.076079358299001186e-06 3.600000000000000000e+01 \\
1.713422646489025329e-06 2.000000000000000000e+01 \\
2.728253397725427844e-06 2.200000000000000000e+01 \\
4.344150941072567507e-06 1.300000000000000000e+01 \\
6.917116795146369262e-06 1.300000000000000000e+01 \\
1.101400605244225566e-05 9.000000000000000000e+00 \\
1.753741232305847315e-05 1.600000000000000000e+01 \\
2.792451988173399519e-05 9.000000000000000000e+00 \\
4.446373251999624366e-05 9.000000000000000000e+00 \\
7.079883621931085927e-05 5.000000000000000000e+00 \\
1.127317687005828983e-04 3.000000000000000000e+00 \\
1.795008555648457756e-04 4.000000000000000000e+00 \\
2.858161237059084073e-04 2.000000000000000000e+00 \\
4.551000958363674910e-04 5.000000000000000000e+00 \\
7.246480518481307606e-04 6.000000000000000000e+00 \\
1.153844624185920622e-03 2.000000000000000000e+00 \\
1.837246941280359491e-03 5.000000000000000000e+00 \\
2.925416691719271399e-03 1.000000000000000000e+00 \\
4.658090661577423200e-03 2.000000000000000000e+00 \\
7.416997610252544504e-03 2.000000000000000000e+00 \\
1.180995767305714934e-02 5.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 1.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 2.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 1.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P2L1 \textit{Ramalingam} (LU)}

\addplot [color=cyan,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 0.000000000000000000e+00 \\
5.355672323345495142e-17 0.000000000000000000e+00 \\
8.527744887236158874e-17 2.000000000000000000e+00 \\
1.357858144994860945e-16 5.000000000000000000e+00 \\
2.162094160073369917e-16 9.000000000000000000e+00 \\
3.442665328668091825e-16 6.200000000000000000e+01 \\
5.481696766070164072e-16 1.400000000000000000e+02 \\
8.728411438927041396e-16 4.130000000000000000e+02 \\
1.389809934740506974e-15 1.006000000000000000e+03 \\
2.212970445101814396e-15 2.001000000000000000e+03 \\
3.523674761908000768e-15 3.395000000000000000e+03 \\
5.610686692716371794e-15 4.790000000000000000e+03 \\
8.933799879640136013e-15 6.205000000000000000e+03 \\
1.422513582750370943e-14 7.466000000000000000e+03 \\
2.265043901107404506e-14 8.172000000000000000e+03 \\
3.606590429895506242e-14 8.174000000000000000e+03 \\
5.742711884151258954e-14 8.048000000000000000e+03 \\
9.144021320249447826e-14 7.495000000000000000e+03 \\
1.455986781017730823e-13 6.719000000000000000e+03 \\
2.318342698746614212e-13 5.889000000000000000e+03 \\
3.691457188282192061e-13 5.143000000000000000e+03 \\
5.877843763257023817e-13 4.288000000000000000e+03 \\
9.359189486181407799e-13 3.663000000000000000e+03 \\
1.490247637846552614e-12 3.068000000000000000e+03 \\
2.372895671560269633e-12 2.513000000000000000e+03 \\
3.778320948218980523e-12 2.059000000000000000e+03 \\
6.016155433569283648e-12 1.690000000000000000e+03 \\
9.579420778937883812e-12 1.431000000000000000e+03 \\
1.525314687647692826e-11 1.174000000000000000e+03 \\
2.428732331571860646e-11 9.220000000000000000e+02 \\
3.867228701193063528e-11 7.690000000000000000e+02 \\
6.157721718824541940e-11 5.780000000000000000e+02 \\
9.804834339067063717e-11 4.750000000000000000e+02 \\
1.561206900965634076e-10 4.030000000000000000e+02 \\
2.485882885252948555e-10 3.360000000000000000e+02 \\
3.958228544449383214e-10 2.810000000000000000e+02 \\
6.302619203438316061e-10 2.200000000000000000e+02 \\
1.003555211061595491e-09 1.690000000000000000e+02 \\
1.597943694741166071e-09 1.440000000000000000e+02 \\
2.544378249864251924e-09 1.110000000000000000e+02 \\
4.051369707010175105e-09 1.020000000000000000e+02 \\
6.450926273935649569e-09 8.700000000000000000e+01 \\
1.027169890709968382e-08 4.800000000000000000e+01 \\
1.635544942815531977e-08 5.900000000000000000e+01 \\
2.604250070181215253e-08 6.200000000000000000e+01 \\
4.146702576306885557e-08 3.100000000000000000e+01 \\
6.602723161356621264e-08 3.300000000000000000e+01 \\
1.051340247902284045e-07 2.600000000000000000e+01 \\
1.674030986681766912e-07 2.100000000000000000e+01 \\
2.665530735613191436e-07 2.100000000000000000e+01 \\
4.244278725438702794e-07 1.000000000000000000e+01 \\
6.758091984659704700e-07 1.300000000000000000e+01 \\
1.076079358299001186e-06 1.500000000000000000e+01 \\
1.713422646489025329e-06 7.000000000000000000e+00 \\
2.728253397725427844e-06 5.000000000000000000e+00 \\
4.344150941072567507e-06 9.000000000000000000e+00 \\
6.917116795146369262e-06 1.000000000000000000e+00 \\
1.101400605244225566e-05 3.000000000000000000e+00 \\
1.753741232305847315e-05 5.000000000000000000e+00 \\
2.792451988173399519e-05 2.000000000000000000e+00 \\
4.446373251999624366e-05 1.000000000000000000e+00 \\
7.079883621931085927e-05 2.000000000000000000e+00 \\
1.127317687005828983e-04 0.000000000000000000e+00 \\
1.795008555648457756e-04 1.000000000000000000e+00 \\
2.858161237059084073e-04 1.000000000000000000e+00 \\
4.551000958363674910e-04 2.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 0.000000000000000000e+00 \\
1.837246941280359491e-03 1.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 1.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 1.000000000000000000e+00 \\
2.994254735955888952e-02 1.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 1.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 0.000000000000000000e+00 \\
1.237229769807379753e+00 0.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P1L2 our}


\addplot [dashed,color=black,line width=2pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.296141396670543711e-18 0.000000000000000000e+00 \\
2.063823643655602038e-18 0.000000000000000000e+00 \\
3.286190876283333322e-18 0.000000000000000000e+00 \\
5.232545187940447735e-18 0.000000000000000000e+00 \\
8.331691668137306856e-18 0.000000000000000000e+00 \\
1.326640928259833440e-17 0.000000000000000000e+00 \\
2.112387523010191339e-17 0.000000000000000000e+00 \\
3.363518305757538773e-17 0.000000000000000000e+00 \\
5.355672323345495142e-17 1.000000000000000000e+00 \\
8.527744887236158874e-17 2.000000000000000000e+00 \\
1.357858144994860945e-16 0.000000000000000000e+00 \\
2.162094160073369917e-16 4.000000000000000000e+00 \\
3.442665328668091825e-16 3.000000000000000000e+01 \\
5.481696766070164072e-16 8.700000000000000000e+01 \\
8.728411438927041396e-16 2.840000000000000000e+02 \\
1.389809934740506974e-15 7.070000000000000000e+02 \\
2.212970445101814396e-15 1.498000000000000000e+03 \\
3.523674761908000768e-15 2.623000000000000000e+03 \\
5.610686692716371794e-15 3.867000000000000000e+03 \\
8.933799879640136013e-15 5.211000000000000000e+03 \\
1.422513582750370943e-14 6.036000000000000000e+03 \\
2.265043901107404506e-14 6.695000000000000000e+03 \\
3.606590429895506242e-14 6.631000000000000000e+03 \\
5.742711884151258954e-14 6.484000000000000000e+03 \\
9.144021320249447826e-14 6.173000000000000000e+03 \\
1.455986781017730823e-13 5.637000000000000000e+03 \\
2.318342698746614212e-13 5.163000000000000000e+03 \\
3.691457188282192061e-13 4.790000000000000000e+03 \\
5.877843763257023817e-13 4.127000000000000000e+03 \\
9.359189486181407799e-13 3.765000000000000000e+03 \\
1.490247637846552614e-12 3.438000000000000000e+03 \\
2.372895671560269633e-12 2.941000000000000000e+03 \\
3.778320948218980523e-12 2.732000000000000000e+03 \\
6.016155433569283648e-12 2.475000000000000000e+03 \\
9.579420778937883812e-12 2.234000000000000000e+03 \\
1.525314687647692826e-11 1.934000000000000000e+03 \\
2.428732331571860646e-11 1.785000000000000000e+03 \\
3.867228701193063528e-11 1.640000000000000000e+03 \\
6.157721718824541940e-11 1.455000000000000000e+03 \\
9.804834339067063717e-11 1.238000000000000000e+03 \\
1.561206900965634076e-10 1.160000000000000000e+03 \\
2.485882885252948555e-10 1.026000000000000000e+03 \\
3.958228544449383214e-10 9.270000000000000000e+02 \\
6.302619203438316061e-10 8.420000000000000000e+02 \\
1.003555211061595491e-09 7.400000000000000000e+02 \\
1.597943694741166071e-09 6.440000000000000000e+02 \\
2.544378249864251924e-09 5.690000000000000000e+02 \\
4.051369707010175105e-09 4.650000000000000000e+02 \\
6.450926273935649569e-09 4.180000000000000000e+02 \\
1.027169890709968382e-08 3.380000000000000000e+02 \\
1.635544942815531977e-08 2.770000000000000000e+02 \\
2.604250070181215253e-08 2.050000000000000000e+02 \\
4.146702576306885557e-08 1.650000000000000000e+02 \\
6.602723161356621264e-08 1.480000000000000000e+02 \\
1.051340247902284045e-07 9.400000000000000000e+01 \\
1.674030986681766912e-07 7.700000000000000000e+01 \\
2.665530735613191436e-07 6.400000000000000000e+01 \\
4.244278725438702794e-07 3.800000000000000000e+01 \\
6.758091984659704700e-07 2.900000000000000000e+01 \\
1.076079358299001186e-06 1.900000000000000000e+01 \\
1.713422646489025329e-06 1.900000000000000000e+01 \\
2.728253397725427844e-06 1.200000000000000000e+01 \\
4.344150941072567507e-06 1.000000000000000000e+01 \\
6.917116795146369262e-06 6.000000000000000000e+00 \\
1.101400605244225566e-05 3.000000000000000000e+00 \\
1.753741232305847315e-05 4.000000000000000000e+00 \\
2.792451988173399519e-05 2.000000000000000000e+00 \\
4.446373251999624366e-05 1.000000000000000000e+00 \\
7.079883621931085927e-05 1.000000000000000000e+00 \\
1.127317687005828983e-04 2.000000000000000000e+00 \\
1.795008555648457756e-04 1.000000000000000000e+00 \\
2.858161237059084073e-04 0.000000000000000000e+00 \\
4.551000958363674910e-04 1.000000000000000000e+00 \\
7.246480518481307606e-04 0.000000000000000000e+00 \\
1.153844624185920622e-03 1.000000000000000000e+00 \\
1.837246941280359491e-03 0.000000000000000000e+00 \\
2.925416691719271399e-03 0.000000000000000000e+00 \\
4.658090661577423200e-03 0.000000000000000000e+00 \\
7.416997610252544504e-03 0.000000000000000000e+00 \\
1.180995767305714934e-02 0.000000000000000000e+00 \\
1.880479239289550505e-02 0.000000000000000000e+00 \\
2.994254735955888952e-02 0.000000000000000000e+00 \\
4.767700294942646411e-02 0.000000000000000000e+00 \\
7.591527143444426473e-02 0.000000000000000000e+00 \\
1.208785804568843769e-01 0.000000000000000000e+00 \\
1.924728837449938279e-01 0.000000000000000000e+00 \\
3.064712609718931446e-01 0.000000000000000000e+00 \\
4.879889154990938449e-01 0.000000000000000000e+00 \\
7.770163534903874458e-01 3.000000000000000000e+00 \\
1.237229769807379753e+00 1.000000000000000000e+00 \\
1.970019673873655286e+00 0.000000000000000000e+00 \\
3.136828429252451755e+00 0.000000000000000000e+00 \\
4.994717933561854117e+00 0.000000000000000000e+00 \\
7.953003423202717137e+00 0.000000000000000000e+00 \\
1.266343050614845112e+01 0.000000000000000000e+00 \\
2.016376249961089684e+01 0.000000000000000000e+00 \\
3.210641207714680689e+01 0.000000000000000000e+00 \\
5.112248750635960448e+01 0.000000000000000000e+00 \\
8.140145720917135463e+01 0.000000000000000000e+00 \\
};
\addlegendentry{P1L2 3Q3}

\legend{}

\end{axis}
